Hierarchical Clustering in ${\Lambda}$CDM Cosmologies via Persistence Energy

In this research, we investigate the structural evolution of the cosmic web, employing advanced methodologies from Topological Data Analysis. Our approach involves leveraging LITE, an innovative method from recent literature that embeds persistence diagrams into elements of vector spaces. Utilizing this methodology, we analyze three quintessential cosmic structures: clusters, filaments, and voids. A central discovery is the correlation between \textit{Persistence Energy} and redshift values, linking persistent homology with cosmic evolution and providing insights into the dynamics of cosmic structures.

==> cosmic-arxiv/relworkCONCISE.tex <==
The surge in high-quality observational data from $\Lambda$CDM simulations has significantly enhanced our grasp of the cosmic web's topology, confirming its web-like structure and spurring interest in its connectivity and complexity \cite{Kelesis2022}. Employing TDA to probe the cosmos is a relatively new but theoretically promising technique. Echoing the persistent homology pipeline used by \cite{Wilding_2021}, our study, detailed in Section \ref{sec:methodology}, adopts a fresh framework to analyze the evolution of the cosmic web.

%Our research marks a significant milestone in the topological analysis of the cosmic web, as we are the first to apply a recent vectorization framework from the literature to this domain. This application not only validates the \textit{Spectral Persistence Homology} framework in a new context but also demonstrates the hierarchical clustering behavior of the cosmos, therefore supporting the $\Lambda$CDM model of the universe. Through our approach, we offer a nuanced perspective on the cosmic web's evolution, employing \textit{persistence energy} of PSs (refer to Section \ref{sec:vectorisation}) as a key analytical tool. This enables  qualitative insights, setting a new precedent for understanding the dynamical behaviour of cosmic structures.

Our research pioneers the use of a recent vectorization framework of TDA in analyzing the cosmic web, validating it in a novel context. This application underscores the hierarchical clustering of cosmic structures, reinforcing the $\Lambda$CDM universe model. We study the evolution  of the \textit{persistence energy} of PSs across different redshifts, offering nuanced insights into the cosmic web's evolution and establishing a new benchmark for comprehending the dynamics of cosmic structures.
